SARA: Selective and Adaptive Retrieval-augmented Generation with Context Compression

Retrieval-augmented Generation (RAG) extends large language models (LLMs) with external knowledge but faces key challenges: restricted effective context length and redundancy in retrieved documents. Pure compression-based approaches reduce input size but often discard fine-grained details essential for factual accuracy. We propose SARA, a unified RAG framework that balances local precision and global knowledge coverage under tight context budgets. SARA combines natural-language text snippets with semantic compression vectors to jointly enhance context efficiency and answer correctness. It represents contexts at two complementary levels: 1) fine-grained natural-language spans that preserve critical entities and numerical values, and 2) compact, interpretable vectors that summarize high-level semantics. An iterative evidence-selection module employs the compression vectors for dynamic reranking of contexts. Across 9 datasets and 5 open-source LLMs spanning 3 model families (Mistral, Llama, and Gemma), SARA consistently improves answer relevance (+17.71), answer correctness (+13.72), and semantic similarity (+15.53), demonstrating the importance of integrating textual and compressed representations for robust, context-efficient RAG.

==> src/limitation.tex <==
\section{Limitations \& Future Work}
\label{app:limitations}

While \method demonstrates strong performance, several open questions suggest promising directions for future work. 

First, although the compression vectors serve as effective summaries and preserve salient factual details (e.g. numbers, organization names), the granularity of retained information varies. 
This uncertainty poses challenges on faithfully interpreting the original context. 
A promising direction is to train a lightweight probing model that estimates the likelihood of accurately recovering key contents from compressed representations, guiding more adaptive compression strategies. 
Another approach is to evaluate fidelity through an \emph{evidence reconstruction step}, where compression vectors are decoded back into text and compared to the original using metrics such as conditional self-information (CSI), token overlap, or embedding similarity. 
One way to ensure compressed representations retain sufficient semantic content is through an \textbf{evidence reconstruction step}, which evaluates whether a set of compression vectors can faithfully recover the original evidence. High reconstruction fidelity suggests that the compression vectors are sufficient. 
% We pass the set of compression vectors through a decoder (the LLM itself) to reconstruct the original textual evidence. This assesses whether the model has learned to interpret and utilize the compressed embeddings effectively. 
% We then compare the reconstructed text to the original evidence using information-theoretic measures, such as conditional self-information (CSI), token-level overlap, or embedding-based similarity. 
% If the original evidence can be reliably reconstructed from the compression vectors, it implies that the tokens capture the essential semantics. In such cases, the evidence can be safely used in compressed form during retrieval-augmented generation (RAG), reducing context length without compromising answer quality. Conversely, if reconstruction fidelity is low, the system falls back to using the original natural language version to preserve critical information.
Second, determining the appropriate number of compression vectors per context remains an open challenge. 
Our current method--assigning one vector per sentence--may not be optimal across all inputs. Future research could explore adaptive mechanisms that tailor the number of vectors to the complexity of the contexts. Lastly, developing mechanisms that predict the number of contexts required for a given query would lead to more context-aware and resource-efficient RAG. Future work can also extend the use of compression vectors beyond generation, exploring their utility in tasks such as document reranking and citation resolution. We also envision applying our framework to specialized domains (e.g., legal or scientific retrieval) where concise yet faithful evidence representation is critical. 





% Future work can explore mechanisms that automatically determines the number of evidence required to answer the question, as well as automatically adjusting the number of compression vectors that can sufficiently represent the semantics in the context.





